OB stars at the lowest Local Group metallicity: GTC-OSIRIS observations of Sextans A

Our aim is to find and classify OB stars in Sextans A, to later determine accurate stellar parameters of these blue massive stars in this low metallicity region $(Z \sim 0.1 \rm Z_{\odot})$. Using UBV photometry, the reddening-free index Q and GALEX imaging, we built a list of blue massive star candidates in Sextans A. We obtained low resolution (R $\sim$ 1000) GTC-OSIRIS spectra for a fraction of them and carried out spectral classification. For the confirmed O-stars we derive preliminary stellar parameters. The target selection criteria and observations were successful and have produced the first spectroscopic atlas of OB-type stars in Sextans A. From the whole sample of 18 observed stars, 12 were classified as early OB-types, including 5 O-stars. The radial velocities of all target stars are in agreement with their Sextans A membership, although three of them show significant deviations. We determined the stellar parameters of the O-type stars using the stellar atmosphere code FASTWIND, and revisited the sub-SMC temperature scale. Two of the O-stars are consistent with relatively strong winds and enhanced helium abundances, although results are not conclusive. We discuss the position of the OB stars in the HRD. Initial stellar masses run from slightly below 20 up to 40 solar masses. The target selection method worked well for Sextans A, confirming the procedure developed in Garcia \& Herrero (2013). The stellar temperatures are consistent with findings in other galaxies. Some of the targets deserve follow-up spectroscopy because of indications of a runaway nature, an enhanced helium abundance or a relatively strong wind. We observe a correlation between HI and OB associations similar to the irregular galaxy IC1613, confirming the previous result that the most recent star formation of Sextans A is currently on-going near the rim of the H\,{\sc I} cavity.

==> TABLES/HR.tex <==

 \begin{table*}[h]
\caption{Stellar parameters adopted for the sample of OB  and the F supergiant stars in the HD diagram.}          
      
\centering        
 \resizebox{15.0cm}{!}{

\begin{tabular}{c |c c c c c c c}     
\hline\hline  
  ID    & SpT      & $M_v$   &  $(B-V)_o$  & $T_{eff}$    & BC      &   log(L /\Lsun)   &   R (\Rsun)    \\
 own    &          &         &             &    [kK]      &         &                   &            \\
\hline


OB326 & O7.5~III((f)) & -5.103 $\pm$ 0.003  & -0.327 $\pm$ 0.002  &  37.40 $\pm$ 7.90   & -3.52 $\pm$ 0.34  &    5.35 $\pm$ 0.15                  & 11.25 $\pm$ 0.59    \\
OB623 & O8 Ib         & -5.193 $\pm$ 0.003  & -0.322 $\pm$ 0.002  &  31.40 $\pm$ 7.90   & -3.00 $\pm$ 0.74  &    5.18 $\pm$ 0.32                  & 13.12 $\pm$ 1.83   \\
OB625 & O9~III?       & -6.044 $\pm$ 0.003  & -0.092 $\pm$ 0.002  &  33.00 $\pm$ 1.00   & -3.15 $\pm$ 0.10  &    5.58 $\pm$ 0.06                  & 18.81 $\pm$ 0.03   \\
OB521 & O9.5~III-V    & -6.287 $\pm$ 0.003  & -0.306 $\pm$ 0.002  &  31.90 $\pm$ 3.80   & -3.05 $\pm$ 0.35  &    5.63 $\pm$ 0.16                  & 21.49 $\pm$ 1.18   \\
OB523 & O9.7~I((f))   & -6.403 $\pm$ 0.003  & -0.326 $\pm$ 0.002  &  29.30 $\pm$ 4.40   & -2.79 $\pm$ 0.44  &    5.58 $\pm$ 0.20                  & 23.94 $\pm$ 1.18   \\ 
OB321 & O9.7~I((f))   & -6.181 $\pm$ 0.003  & -0.309 $\pm$ 0.002  &  26.30 $\pm$ 4.3    & -2.48 $\pm$ 0.88  &    5.36 $\pm$ 0.37                  & 23.16 $\pm$ 3.98   \\
OB622 & B0~I          & -6.399 $\pm$ 0.003  & -0.222 $\pm$ 0.002  &  27.80 $\pm$ 1.04   & -2.76 $\pm$ 0.01  &    5.56 $\pm$ 0.02                  & 26.06 $\pm$ 1.34   \\
OB524 & B0~III        & -4.830 $\pm$ 0.003  & -0.293 $\pm$ 0.002  &  27.80 $\pm$ 1.04   & -2.76 $\pm$ 0.01  &    4.93 $\pm$ 0.02                  & 12.65 $\pm$ 0.67   \\
OB222 & B1 I          & -7.008 $\pm$ 0.003  & -0.324 $\pm$ 0.002  &  22.63 $\pm$ 1.04   & -2.27 $\pm$ 0.01  &    5.61 $\pm$ 0.02                  & 41.71 $\pm$ 2.92   \\
OB421 & B1 I          & -6.556 $\pm$ 0.003  & -0.284 $\pm$ 0.002  &  22.63 $\pm$ 1.04   & -2.27 $\pm$ 0.01  &    5.43 $\pm$ 0.02                  & 33.88 $\pm$ 2.37   \\
OB422 & B1 I          & -6.126 $\pm$ 0.003  & -0.304 $\pm$ 0.002  &  22.63 $\pm$ 1.04   & -2.27 $\pm$ 0.01  &    5.26 $\pm$ 0.02                  & 27.79 $\pm$ 1.94   \\
OB323 & B1~III        & -6.316 $\pm$ 0.003  & -0.282 $\pm$ 0.002  &  22.63 $\pm$ 1.04   & -2.27 $\pm$ 0.01  &    5.34 $\pm$ 0.02                  & 30.32 $\pm$ 2.12   \\
OB221 & B2.5 I        & -6.904 $\pm$ 0.003  & -0.229 $\pm$ 0.002  &  17.57 $\pm$ 1.04   & -1.63 $\pm$ 0.01  &    5.32 $\pm$ 0.02                  & 49.14 $\pm$ 4.74   \\
OB324 & B8~II         & -5.320 $\pm$ 0.003  & -0.136 $\pm$ 0.002  &  12.49 $\pm$ 1.04   & -0.77 $\pm$ 0.01  &    4.34 $\pm$ 0.02                  & 31.53 $\pm$ 4.56   \\
OB121 & B8~III        & -7.284 $\pm$ 0.003  & -0.093 $\pm$ 0.002  &  12.49 $\pm$ 1.04   & -0.77 $\pm$ 0.01  &    5.12 $\pm$ 0.02                  & 77.89 $\pm$ 11.27   \\  
OB122 & B9 I          & -7.624 $\pm$ 0.003  & -0.173 $\pm$ 0.002  &  11.46 $\pm$ 1.04   & -0.58 $\pm$ 0.01  &    5.18 $\pm$ 0.02                  & 98.91 $\pm$  15.80  \\
OB621 & F5~I          & -7.670 $\pm$ 0.003  &  0.320 $\pm$ 0.002  &   6.37 $\pm$ 1.04   & -0.03 $\pm$ 0.01  &    4.98 $\pm$ 0.02                  & 254.13 $\pm$ 76.31  \\


% NOPONER: Temperatures derived from spectrocopic analysis values for O program stars and from \citet{Markova08} for B-type stars (with a $\pm$ 1Kk of uncertainty). Bolometric corrections (BC) from the expressions proposed by \citet{Martins05}for O-type stars and \citet{Balona94} for later types. The typical uncertainties on our data are aproximately $\pm$1 kK in temperature and $\pm$ 0.001 mag in the photometry. The deduced errors are: $\pm$0.05 for absolute magnitude, $\pm$0.01 for intrinsic color, lower than $\pm$0.09 for the bolometric correction and $\pm$0.003 for Q parameter. Luminosity and radio derived erros are shown in Table \ref{T:final_results}.

  
\hline
\end{tabular}
 }
\label{T:final_results}
\end{table*} 

